New Physics Signals of the Electroweak Chiral Lagrangian in Vector Boson Scattering at the LHC

The Standard Model of fundamental interactions, albeit an incredibly elegant and successful theory, lacks explanations for some experimental and theoretical open questions. Interestingly, many of these problems seem to be related to the electroweak symmetry breaking sector of the theory, whose dynamical generation is still unknown. Important questions such as what is the true nature of the Higgs boson, why is its mass so light and so close to that of the electroweak gauge bosons or whether the properties of this particle are the ones predicted in the Standard Model remain unanswered. The LHC is our tool to unveil these mysteries and vector boson scattering processes are the perfect window to access them, since they are considered as the most sensitive observables to new physics in the electroweak symmetry breaking sector. In this Thesis we employ the effective electroweak chiral Lagrangian with a light Higgs, which assumes a strongly interacting electroweak symmetry breaking sector, to perform a model independent analysis of the phenomenology of vector boson scattering processes at the LHC as well as to present quantitative predictions for the sensitivity to possible beyond the Standard Model physics scenarios.

==> Publicaciones/Publicaciones_old.tex <==

\thispagestyle{empty}
\begin{center}
	\Large {\bfseries\scshape List of Publications}\\[-8pt]
	 {\color{col1}\rule{6cm}{0.8mm}}
	\vspace{0.5cm}
%	\vspace{1cm}
\end{center}



	%%%%%%%%%%%%%%%%%%
	% Bloc rubriques %
	%%%%%%%%%%%%%%%%%%
% \begin{flushleft}
%\vspace{-1cm}
\justifying

%{\large \underline{Publications in International Journals}}
%\vspace{0.2cm}

This Thesis is based on the following scientific articles:

\newlist{coloritemize}{itemize}{1}
\setlist[coloritemize]{label=\textcolor{color1}{\textbullet}}

\begin{coloritemize}

 \item {\bfseries Probing the Higgs self-coupling in double Higgs production through vector boson scattering at the LHC  } \\
  E. Arganda, C. Garcia-Garcia, M. J. Herrero  \\ 
   \href{https://www.sciencedirect.com/science/article/pii/S0550321319301737?via\%3Dihub}{\textbf{DOI: 10.1016/j.nuclphysb.2019.114687} }
   [\href{https://arxiv.org/pdf/1807.09736}{\textbf{arXiv:1807.09736}}].

\vspace*{0.2cm}

 \item { \bfseries Unitarization effects in EFT predictions of WZ scattering at the LHC} \\
  C. Garcia-Garcia, M. J. Herrero, R. Morales \\
   %\href{http://iopscience.iop.org/article/10.1088/1475-7516/2018/06/031/meta}{\textbf{DOI:cambiar} }
   $[$\href{https://arxiv.org/abs/1907.06668}{\textbf{arXiv:1907.06668}}$]$.

\vspace*{0.2cm}

 \item {\bfseries Production of vector resonances at the LHC via $\boldsymbol{WZ}$-scattering: a unitarized EChL analysis} \\
  R. L. Delgado, A. Dobado, D. Espriu, C. Garcia-Garcia, M. J. Herrero, X. Marcano, J. J. Sanz-Cillero \\ 
   \href{https://link.springer.com/article/10.1007\%2FJHEP11\%282017\%29098}{\textbf{DOI: 10.1007/JHEP11(2017)098} }
   [\href{https://arxiv.org/pdf/1707.04580}{\textbf{arXiv:1707.04580}}].
   
   
\vspace*{0.2cm}

 \item {\bfseries Dynamical vector resonances from the EChL in VBS at the LHC: the WW case} \\
  R. L. Delgado, C. Garcia-Garcia, M. J. Herrero \\ 
   %\href{https://link.springer.com/article/10.1007\%2FJHEP11\%282017\%29098}{\textbf{DOI: cambiar} }
   $[$\href{https://arxiv.org/pdf/1907.11957}{\textbf{arXiv:1907.11957}}$]$.
   
\end{coloritemize}
   
 and conference proceedings:
   
\begin{coloritemize}

 \item {\bfseries Collider phenomenology of vector resonances in WZ scattering processes} \\
  R. L. Delgado, A. Dobado, D. Espriu, C. Garcia-Garcia, M. J. Herrero, X. Marcano, J. J. Sanz-Cillero \\ 
   Conference proceeding, $[$\href{https://arxiv.org/abs/1811.08720}{\textbf{arXiv:1811.08720}}$]$.
   
   
\vspace*{0.2cm}

 \item {\bfseries Resonant $\boldsymbol{pp \to W^+Zjj}$ events at the LHC from a unitarized study of the EChL} \\
  R. L. Delgado, A. Dobado, D. Espriu, C. Garcia-Garcia, M. J. Herrero, X. Marcano, J. J. Sanz-Cillero\\ 
   Conference proceeding, $[$\href{https://arxiv.org/abs/1805.04870}{\textbf{arXiv:1805.04870}}$]$.


\end{coloritemize}






